Iso-Points: Optimizing Neural Implicit Surfaces with Hybrid Representations

Neural implicit functions have emerged as a powerful representation for surfaces in 3D. Such a function can encode a high quality surface with intricate details into the parameters of a deep neural network. However, optimizing for the parameters for accurate and robust reconstructions remains a challenge, especially when the input data is noisy or incomplete. In this work, we develop a hybrid neural surface representation that allows us to impose geometry-aware sampling and regularization, which significantly improves the fidelity of reconstructions. We propose to use \emph{iso-points} as an explicit representation for a neural implicit function. These points are computed and updated on-the-fly during training to capture important geometric features and impose geometric constraints on the optimization. We demonstrate that our method can be adopted to improve state-of-the-art techniques for reconstructing neural implicit surfaces from multi-view images or point clouds. Quantitative and qualitative evaluations show that, compared with existing sampling and optimization methods, our approach allows faster convergence, better generalization, and accurate recovery of details and topology.

==> 04-method.tex <==
% !TeX root = ./DSS2.tex
\section{Method}\label{sec:method}
\begin{figure}
\includegraphics[width=\linewidth, trim={0 1cm 0 0}, clip]{figures/overview}
\caption{Overview of our implicit-explicit representation. We efficiently extract a dense uniformly distributed point cloud, \emph{iso-points}, as an explicit representation for a neural implicit surface. As the extraction is fast, iso-points can be integrated back into the optimization as a 3D geometric prior, enhancing the optimization.}\label{fig:overview}
\end{figure}
%, \eg guide efficient sampling of the training data and enable additional regularization.

%An implicit function represents the surface $ \S $ of a shape as the zero level set of a function $ s = f(\p)$, where $ \p\in \R^3 $ denotes a point in the 3D space and $ s \in \R$ is typically the signed distance value of the point.
%An explicit representation can be extracted by the marching cube algorithm \cite{}, which exhaustively evaluates the function $ f $ on a 3D grid, then extracts the surface mesh based on the sign changes between the neighboring grid points.
%Due to the prohibiting computational cost of marching cube, explicit representations have been so far entirely neglected during the training phase.
%However, as we demonstrate in Section~\ref{sec:result} having an explicit representation during the training phase have a significant role in improving the convergence rate, reconstruction quality and optimization robustness.
%
Given a neural implicit function $ f(\p;\theta_t) $ representing surface $ \S_t $, where $ \theta_t $ is the network parameters at the $t$-th training iteration, our goal is to efficiently generates a dense and uniformly distributed point set on the zero level set, called \emph{iso-points}, which faitfully represents the current implicit surface $ \S_t $.
Intuitively, we can deploy the iso-points back in the ongoing optimization to serve various purposes, \eg improving the sampling of training data and providing regularization for the optimization, leading to a substantial improvement in the convergence rate and the final optimization quality.

In this section, we first focus on how to extract the iso-points via projection and uniform resampling. We then explain how to utilize the iso-points for better optimization in practical scenarios.

\subsection{iso-surface sampling}
As shown in Figure~\ref{fig:overview}, our iso-surface sampling consists of three stages. 
First, we project a set of initial points $ \Q $ onto the zero level set to get a set of \emph{base iso-points} $ \tilde{\Q} $.
Then we resample $ \tilde{\Q} $ to avoid points clustering and fill large holes.
Finally, we upsample the points to obtain dense and uniformly distributed iso-points $ \P_t $.

\paragraph{Projection.} Projecting a point onto the iso-surface can be seen as performing newton-method~\cite{ben1966newton} to approximate the root of the function starting from the given point.
Atzmon \etal~\cite{atzmon2019controlling} derived the projection formula for functions modeled by generic purposed networks.
For completeness, we recapitulate the steps here, focusing on $ f:\R^3\to\R $.

Given an implicit function $ s=f(\p) $ representing the signed distance field and an initial point $ \q_0 $, we can find an iso point $ \p $ iteratively using newton-method
$ \q_{k+1} = \q_{k} - J_f(\q_{k})^{+}f(\q_{k})$,  where $  J_f^{+} = (J_f^T J_f)^{-1} J_f^T$ is the Moore-Penrose pseudo-inverse of the Jacobian. 
In our case, $ J_f$ is a 1 by 3 vector, $  J_f^{+}(\q_{k}) =\frac{J_f^T(\q_{k})}{\|J_f(\q_{k})\|^2} $
%\begin{equation}\label{eq:newton}
%\q_{k+1} = \q_{k} - \frac{J_f^T(\q_{k})}{\|J_f(\q_{k})\|^2}f(\q_{k}),
%\end{equation}
where the Jacobian $ J_f(\q_{k}) $ can be conveniently evaluated in the network via back-propagation.

However, for some contemporary network designs, such as sinus activation function~\cite{sitzmann2020implicit} and positional encoding~\cite{mildenhall2020nerf}, the signed distance field can be very noisy, and the gradient highly unsmooth.
Directly applying the newton-method will cause overshooting and oscillation. 
%The success rate of the projection is significantly low.
While one could apply more sophisticated line-search algorithm, we address this issue with a simple clipping operation to bound the length of update, \ie
\begin{equation}\label{eq:projection}
	\q_{k+1} = \q_{k} - \tau(\frac{J_f^T(\q_{k})}{\|J_f(\q_{k})\|^2}f(\q_{k})),
\end{equation}
where $ \tau(\vec{v}) = \frac{\vec{v}}{\|\vec{v}\|}\min(\|\vec{v}\|, \tau_0) $ bounds the length of the update. 
We set $ \tau_0=\frac{D}{2|\Q|} $ with $ D $ denoting the diagonal length of the input shape.

In practice, we initialize $ \Q_t $ with a unit sphere shape at the beginning of the training and then with iso-points $ \P_{t-1} $ from the previous training iteration.
Similar to \cite{atzmon2019controlling}, we perform the projection step a maximum of 10 times at each training iteration until all the points have converged, \ie $ f(\q_{k}) < \epsilon, \forall \q \in \Q$. In our experiments, the termination threshold $ \epsilon $ is set to $ 10^{-4}  $ at the beginning of the training then is gradually reduced to $10^{-5} $.


\paragraph{Upsampling.}
The resampling step generates a sparse point cloud that is free from large holes and points clustering.
Next, we upsample the point set to the desired density while further improving the point distribution.

Our upsampling step is based on edge-aware resampling (EAR) proposed by Huang \etal\cite{huang2013edge}.
% which preserves sharp geometry features by separating points on either side of the edge then progressively inserting points close to the edges.
%This desirable in our case since sharp features are usually under-sampled after projection.
Here, we explain the key steps of and our main differences to EAR.

First, we apply bilateral normals filtering, the same as in EAR.
%\begin{equation}\label{eq:ear-normal}
%	\n = \dfrac{\sum_{\p_i\in \N(\p)}w(\p_i, \p)\psi(\n_i, \n)\n_i}{\sum_{\p_i\in \N(\p)}w(\p_i, \p)\psi(\n_i, \n)},
%\end{equation}
%where $ \psi(\n_i, \n)=e^{-(1-\frac{1-\n_i^T\n}{1-\cos(\sigma_n)})} $ $ w(\p_i, \p) $ is the spatial weight in \eqref{eq:repulsion_direction}.
Then, the points are pushed away from the edge to create a clear separation. 
We simplify the original optimization formulation with a simpler update, divided into an attraction term and a repulsion term.
The former pulls points away from the edge and the latter prevents the points from clustering.
\begin{align}\label{eq:ear-push}
\Delta\p_{\text{attraction}} &= \dfrac{\sum_{\p_i\in \N(\p)}\phi(\n, \p_i - \p)(\p-\p_i)}{\sum_{\p_i\in \N(\p)}\phi(\n, \p_i - \p)} \\
\Delta\p_{\text{repulsion}} &= 0.5\dfrac{\sum_{\p_i\in \N(\p)}w(\p_i,\q)(\p_i - \p)}{\sum_{\p_i\in \N(\p)}w(\p_i,\q)} \\
\p & \leftarrow \p - \tau(\Delta\p_{\text{repulsion}}) - \tau(\Delta\p_{\text{attraction}}),
\end{align}
where $ \phi(\n, \p - \p_i) = e^{-(\n_i^T(\p - \p_i))^2/\sigma_p} $ is the anisotropic projection weight and $ w $ is the spatial weight defined in \eqref{eq:spatial_w}.
We use directional clipping function $ \tau $ as before to bound the two update terms individually, which improves the stability of the algorithm for sparse point cloud.

In the insertion step, new points are inserted in sparse areas or sharp boundaries. 
The trade-off is controlled by a unifying priority score $ P(\p) = \max_{\p_i\in\N(\p)}B(\p, \p_i) $, where $ B $ is a distance measure (see \cite{huang2013edge} for the exact definition).
%In the insertion step, for each point $ \p $, a set of insertion candidates $\vec{b}_i=b(\p_i, \p)$ are proposed from every neighbor in its neighborhood $ \p_i\in\N(\p) $.
%The insertion prioritize sparse areas or sharp boundaries, which is indicated by a priority score $ P(\p) = \max_{\p_i\in\N(\p)}(1-\n^T_i\n)^\rho C(\vec{b}_i) $, 
%where $ C(\vec{b}_i) $ is the minimum distance between the candidate $ \vec{b}_i $ and all other neighboring points in the neighborhood (we refer to \cite{huang2013edge} for the definition of the distance) and $ \rho $ is a parameter indicating edge-sensitivity, larger $ \rho $ prioritizes insertion close to edges.
Denoting the point with maximum priority as $ \p^* $, a new point is inserted at the midpoint between $ \p^* $ and neighbor $ \p^*_{i^*} $ where $ \p^*_{i^*}=\arg\max_{\p_i\in\N(\p^*)} B(\p^*, \p_i) $.
In the original work, the insertion is done iteratively, requiring an update of the neighborhood information and recalculation of $ B $ after every insertion.
Instead, we approximate this process by adding a maximum of $ |\P|/10 $ points each step.
However, since the point and its neighbors are likely to be selected together, inserting the new point at the midpoint would lead to overlapping.
Thus we insert asymmetrically at $ (\p^*_{i^*}+2\p^*)/3 $ instead.

After the resampling and upsampling, we perform another aforementioned projection-step to ensure the dense iso-points lie on the zero level set surface.

Compared with using marching cubes to extract the iso-sufrace at each iteration, our adaptive sampling is efficient. Since both the resampling and upsampling steps only require local point statistics, we implement it on GPU.
Furthermore, since we use the iso-point from the last iteration for initialization, the overall points distribution improves as the training stabilizes, requiring fewer (or even zero) resampling and upsampling steps at later stages.
%Since the resulting point cloud from the resampling and upsampling step already lie close to the surface, the final projection step does not create artifacts.
As shown in Figure~\ref{fig:overview}, the final iso-points faithfully mirrors the 3D geometry of the current implicit surface.

\subsection{Utilizing iso-points in optimization}\label{sec:method-application}

%
%\begin{figure}
%	\includegraphics[width=1.0\linewidth]{figures/2D_sampling}
%	\caption{A 2D illustration of training samples generated via ray-marching (left) and from uniformly distributed iso-points (right). With iso-points, the samples are more evenly distributed on the entire surface and areas with higher curvature is less likely to be under-represented.}\label{fig:2D_sampling}
%\end{figure}

\subsubsection{iso-points for importance sampling}\label{sec:method-sampling}
Optimizing a neural implicit function to represent a high-resolution 3D shape requires abundant training samples. 
In particular, more samples are required close to the surface to accurately capture the fine-grained geometry details. 
However, for applications where the explicit 3D geometry is not available during training, how to generate training samples remains mostly unexplored.
For example, in multi-view reconstruction, existing works \cite{niemeyer2020differentiable, yariv2020multiview} randomly sample pixels on the input image, then use variants of ray-tracing to obtain 3D sample points. 
Such approach leads to undersampling on small-scaled geometric details.

\begin{figure}\centering
	\includegraphics[width=\linewidth]{figures/distribution}
	\caption{Examples of importance sampling based on different saliency metrics. The default uniform iso-points represent different regions of the iso-surface equally. We compute different saliency metrics on the uniform iso-points, based on which more samples can be inserted to highlight salient regions. The curvature-based metric emphasizes geometric details estimated from current surface prediction, while the loss-based metric hard examples.}\label{fig:metric_sampling}
\end{figure}
Since iso-points provide an explicit representation of the 3D shape, we can naturally use them to generate samples more densely on the current iso-surface.
More specifically, for each view in the training batch, we use a point rasterizer to efficiently determine the subset of visible iso-points, then project this subset onto the image to obtain the ground truth visibility and color intensity.

More importantly, iso-points allows us to draw samples adapted to the approximated 3D geometry features and the current state of the training.
The main idea is to compute a saliency metric on each iso-point, then in the next training step insert more samples in the neighborhood high saliency.
To this end, we experiment two types of metrics, curvature-based and loss-based.
The former is motivated to emphasis the geometric features which are typically reflected by high curvature, while the latter is a form of hard example mining as we aim to sample more densely where higher loss occurs.

Since the iso-points are uniformly distributed, the curvature can be approximated by the norm of Laplacian, \ie $ \mathcal{R}_{\text{curvature}}(\p) = \|\p-\sum_{\p_i\in\N(\p)} \p_i\| $.
For the loss-based metric, we project the iso-points on all training views and compute the average loss on each point, \ie $ \mathcal{R}_{\text{loss}}(\p) = 1/N\sum_{i}^{N} \text{loss}(\p)$, where $ N $ is the number of occurrences of $ \p $ in all views.

As both metrics evolve smoothly and remain consistent during the training, we need not update them in each iteration.
Denoting the iso-points on which we computed the metric as $ \mathcal{T} $ and the subset of template points with high metric values $ \mathcal{T}^*=\{\vec{\vec{t}^*}\} $, the metric-based insertion for each point $ \p $ in the current iso-points $ \P_t $ can be written as
\begin{equation}\label{key}
\p_{\text{new},i} = 2/3\p + 1/3\p_i, \forall \p_i \in \N(\p), \;\text{if } \min_{\vec{t}^*}\|\p-\vec{t}^*\|\leq \sigma.
\end{equation}
The neighborhood $ \sigma $ is the same one used to compute the weight in \eqref{eq:repulsion_direction}.

An example of the sampling result for both metrics is shown in Figure~\ref{fig:metric_sampling}.

\subsubsection{iso-points for regularization}\label{sec:method-reg}
The direct access to an explicit representation of the 3D surface also enables us to incorporate geometry-motivated priors into the optimization objective, exerting finer control of the reconstruction result.
\begin{figure}\centering
	\includegraphics[width=0.3\linewidth]{figures/smoothness00_L03}
	\includegraphics[width=0.3\linewidth]{figures/smoothness00_L02}
	\includegraphics[width=0.3\linewidth]{figures/smoothness00_L05}
\caption{Progression of overfitting. When optimizing a neural implicit function from noisy point cloud, the network initially outputs a smooth surface, but increasingly overfits to the noise in the data. Shown here are the reconstructed surface after 1000, 2000 and 5000 iterations.}\label{fig:overfitting}
\end{figure}
\begin{figure}\centering
\includegraphics[width=0.3\linewidth]{figures/toy00}
\includegraphics[width=0.3\linewidth]{figures/toy02}
\includegraphics[width=0.3\linewidth]{figures/toy01}
\caption{Iso-points for regularization. At the early stage of the training, the implicit surface is smooth (left), we extract iso-points (middle) as a reference shape, which can facilitate various regularization terms. In the example on the right, we use the iso-points to detect outliers in the training data (shown in red).}\label{fig:reg}
\end{figure}

Let us consider fitting a neural implicit surface from a point cloud.
Depending on the acquisition process, the point cloud may be sparse, distorted by noise or distributed highly unevenly.
Similar with previous works \cite{ulyanov2018deep, williams2019deep} in image and explicit surface reconstruction, we observe that the network tends to first fit a smooth surface from these corrupted observation, but then as the network starts to pick up higher-frequency signals from the data, it also starts to overfit to noise and other caveats in the data as shown in Figure~\ref{fig:overfitting}.
Moreover this characteristic is consistent across network architectures, including those that are designed to accommodate high-frequency information such as SIREN.
Existing methods that addresses overfitting include early stopping, weight decay and drop-out \etc\cite{goodfellow2016deep}.
However, whereas these methods are generic tools designed to improve network generalizability for training large dataset, we propose a novel regularization approach that is specifically tailored for training neural implicit surfaces and serve as a platform to integrate a plethora of 3D priors from classic geometry processing.

Our main idea is to use the iso-points as a consistent, smooth but dynamic approximation of the reference geometry.
Consistency and smoothness is to ensure that the optimization does not fluctuate and overfit to noise, at the same time the dynamic nature lets the network pick up consistent high frequency signals governed by underlying geometry details.
To this end, we propose to start extracting iso-points after a short warmup training (\eg 300 iterations) and update the iso-points periodically (\eg every 1000 iterations).
Thanks to the aforementioned smooth characteristic of the network, the extracted iso-points are smooth.
The period update allows the iso-points to evolve as the network learns more high-frequency information but ensures the change is coherent and stable.

The utility of the reference geometry includes but not limited to
\begin{inparaenum}[1)]
\item as additional training data to circumvent data scarcity, 
\item enforce additional geometric constraints,
\item filter outliers in the training data.
\end{inparaenum}

Specifically, for sparse or hole-ridden input point cloud, we take advantage of the uniform distribution of iso-points and augment supervision in undersampled areas by enforcing the SDF value on all iso-points to be zero, \ie
\begin{equation}\label{eq:iso_sdf}
\mathcal{L}_{\text{isoSDF}} = \dfrac{1}{|\P|}\sum_{\p\in \P}|f(\p)|.
\end{equation}

Given the iso-points, we compute their normals from their local neighborhood using Principal Component Analysis (PCA). 
Then we increase surface smoothness by enforcing consistency between the normals estimated by PCA and those from the gradient of the network, \ie
\begin{equation}\label{eq:iso_normal}
\mathcal{L}_{\text{isoNormal}} = \dfrac{1}{|\P|}\sum_{\p\in \P}(1-|\cos(J_f^T(\p), \n_{\text{PCA}})|).
\end{equation}
The larger PCA neighborhood is, the smoother the reconstruction becomes.
Optionally, if desired, additional normal filtering can be applied after PCA to reduce over-smoothing and enhance geometric features.

Last but not least, the iso-points can be used filter outliers in the training data.
Specifically, given a batch of training points $ \Q=\{\q\} $, we compute a per-point loss weight based on their alignment with the iso-points.
We choose to use bilateral weights so as to take the euclidean and directional distance both into consideration.
Denoting the normal of an iso-point $ \p $ and a training point $ \q $ as $ \n_\p $ and $ \n_\q $, the bilateral weight can written as
\begin{align}
v(\q)  = \min_{\p\in\P}w(\p, \q)\psi(\n_\p, \n_\q),\quad \text{with}\\\label{eq:outlier_weight}
\psi(\n_\p, \n_\q) =e^{-\left(1-\frac{1-\n_\p^T\n_\q}{1-\cos\left(\sigma_n\right)}\right)^2},
\end{align}
where $ \sigma_n $ indicating the sensitivity to normal difference, we set $ \sigma_n = 60^\circ $ in our experiments.
This loss weight can be incorporated into the existing loss functions to reduce the impact of outliers in the data.
A visualization of the outliers detected by this weight is shown in Figure~\ref{fig:reg}.



==> 05-results.tex <==
% !TeX root = ./DSS2.tex
\begin{figure}
	\includegraphics[width=\linewidth]{figures/ray-tracing}
	\caption{A 2D illustration of two sampling strategies for multi-view reconstruction. Ray-tracing (left) generates training samples by shooting rays from the camera $ \mathcal{C} $ through randomly sampled pixels, depending on whether an intersection can be found and whether the pixel lies inside the object silhouette, three types of samples are generated -- on-surface, in-surface and out-surface points. Instead, we generate on-surface samples directly from iso-points, which provide evenly distributed samples on the implicit surface. We also use the iso-points to generate more reliable in-surface samples. }\label{fig:ray-march}
\end{figure}
\section{Results}\label{sec:result}
The iso-points can be incorporated into the optimization pipelines of existing state-of-the-art methods for implicit surface reconstruction.
In this section, we demonstrate the benefits of the specific techniques introduced in Section~\ref{sec:method-sampling} and Section~\ref{sec:method-reg}.

We choose a state-of-the-art method as the baseline for each experiment, then augment the optimization with iso-points.
Results show that the augmented optimization outperforms the baseline quantitatively and qualitatively.

\subsection{Sampling with iso-points.}
We evaluate the benefit of utilizing iso-points to generate training samples for multi-view reconstruction.
%We focus on multi-view reconstruction, since the advantage of an explicit 3D representation is particularly pronounced in these cases where no 3D information is available.

\begin{table}\centering\small
	\begin{tabular}{lcc}
		\toprule
		& \makecell[c]{chamfer $ 10^{-4} $ \\ (position)} & \makecell[c]{chamfer $ 10^{-2} $ \\ (normal)}\\\midrule
		baseline (ray-tracing) & 1.439 & 5.987 \\
		%\multicolumn{3}{c}{\textit{alternatives}}\\
%		\makecell[c]{\textit{alternatives}} & &\\
		+ uniform iso-points & 1.405 & 5.404 \\
		+ loss-based iso-points & \textbf{1.081} & \textbf{4.121} \\
		+ curvature-based iso-points & 1.489 & 5.948 \\
%		image-saliency-based & 2.329 & 7.970 \\
		%ray-tracing & 1.438505860278383 & 0.05986650288105011 \\
		%+ uniform iso-points & 1.4049177116248757 & 0.05404352396726608\\
		%+ curvature iso-points & 1.4885226846672595 & 0.059485167264938354\\
		%+ loss-based iso-points & 1.0807582293637097& 0.04120780527591705\\
		\bottomrule
	\end{tabular}
	\caption{Quantitative effect of importance sampling with iso-points. All methods use the same amount of optimization time. Compared to the baseline, which generates training points via ray-marching through randomly sampled pixels, we use iso-points to draw more attention on the implicit surface.}\label{tab:sampling}
\end{table}

As the baseline, we implement the ray-tracing algorithm from IDR \cite{yariv2020multiview}, which generates training samples by ray-marching from the camera center through uniformly sampled pixels on the image.
As shown in Figure~\ref{fig:ray-march}, three types of samples are used for different supervisions: on-surface samples, which are ray-surface intersections inside the object's 2D silhouette; in-surface samples, which are points with the lowest signed distance on the non-intersecting rays inside 2D silhouette; and out-surface samples, which are on the rays outside the 2D silhouette either at the surface intersection or at the position with the lowest signed distance. 
% Depending on whether an intersection can be found on the ray, the training points are divided into on-surface points and off-surface points, which are supervised by the pixel color and the silhouette of the object respectively.
%To accommodate the irregularities of the signed distance field during training, the ray-marching algorithm (illustrated in Figure~\ref{fig:ray-march} left) is an expensive operation involving \begin{inparaenum}[1)]
%	\item find the intersections with a bounding sphere,
%	\item perform sphere-trace bidirectionally from both intersections,
%	\item approximate a root of the implicit function, as an ``on-surface" sample, using secant-method in the range determined by the sphere tracing.
%\end{inparaenum}
%If no intersections can be found, an in-surface sample (or out-surface, depending on the silhouette of the object) is generate on the ray, which is chosen as the point with the lowest signed-distance value on the ray and is aimed to provide supervision on the visual hull of the implicit surface by comparing against with the silhouette of the object.
%\yf{too complicated to explain, need an illustration.}

On this basis, we incorporate the iso-points directly as on-surface samples and optionally control the optimization focus by varying the iso-points distribution using the saliency metrics as described in Section~\ref{sec:method-sampling}, and a 3D prior to generate more reliable in-surface samples behind the iso-points.
More specifically, as shown in Figure~\ref{fig:ray-march} right, we generate the three types of samples as following:
\begin{inparaenum}[a)]
\item on-surface samples: filter iso-points by visibility using a point rasterizer, then choose the iso-points whose projections are inside the object silhouette;
\item in-surface samples: on the camera rays which pass through the on-surface samples, choose the point with the lowest signed distance on the segment between the on-surface sample and the farther intersection of the object's bounding sphere.
\item out-surface samples: shoot camera rays through pixels outside the object silhouette, choose the point with the lowest signed distance.
\end{inparaenum}

Below, we demonstrate two benefits of the proposed sampling scheme separately.
\begin{figure*}[h!]
	\centering
	{\includegraphics[width=1.\linewidth]{figures/compressor3.png}}
	\caption{Qualitative comparison between sampling strategies for multi-view reconstruction. Under the same optimization time and similar total sample count, sampling the surface points with uniformly distributed iso-points improves the reconstruction accuracy considerably. The result can be further enhanced with a loss-based importance sampling. \yf{change figure text to ray-tracing, uniform iso-points, loss-based iso-points, reference?}}
	\label{fig:compressor}
\end{figure*}
\paragraph{Surface details from importance sampling.} 
First, we examine the effect of drawing on-surface samples using iso-points by comparing the optimization results under fixed optimization time (100 minutes) and total sample count.

%To limit other interfering factors such as unknown lighting and insufficient views, 
We create a synthetic dataset with known lighting and material and render $ 512\times512 $ images per object from varied camera positions.
When training with the iso-points, we extract 4000 iso-points after 100 iterations then increase the density by 1.2 times every 800 iterations until reaching 15000 points.
To match the sample count, in the ray-tracing variation we randomly draw 2048 pixels per image then increase by 1.2 times per 800 iterations until reaching 10000 pixels.
We use a 3-layer SIREN model with the frequency multipliers set to 30, and optimize with a batch size of 4.

Table~\ref{tab:sampling} summarizes the quantitative comparison of the reconstructed surface for the compressor model shown in Figure~\ref{fig:compressor} (first row).
We compute 2-way chamfer point-to-point distance ($ \|\p_i - \p_j\|^2 $) and normal distance ($1- \cos(\vec{n}_i, \vec{n}_j) $) on 50K points uniformly sampled from the reconstructed meshes.
%Both the squared euclidean distance ($ \|\p_i - \p_j\|^2 $) and the normal discrepancy ($1- \cos(\vec{n}_i, \vec{n}_j) $) are measured.
Using uniform iso-points as on-surface samples compares favorably against the baseline, especially in the normal metrics, indicating higher fidelity on the finer geometry features as the surface samples overcome under-sampling issues occurring at small-scale geometry details.
Importance sampling with iso-points and loss-based upsampling shows a substantial advantage over other variations, demonstrating the effectiveness to allocate the training samples based on current optimization state.
In comparison, the curvature-based sampling performs similarly to the baseline, but notability worse than with the uniform iso-points.
We observe the iso-points in this case are highly concentrated on few spots on the surface, but ignored regions where the current reconstruction is actually problematic (Figure~\ref{fig:metric_sampling}), which may be the reason for the weaker performance.
%For completeness, we also compare an alternative importance sampling strategy based on the image laplacian

The improvement is more pronounced qualitatively as shown in Figure~\ref{fig:compressor}.
Using uniform iso-points for on-surface samples clearly enhances reconstruction fidelity compared to the baseline with ray-tracing.
The finer geometric details further improved with loss-based importance sampling.

\paragraph{Topological correctness from 3D prior.}
\begin{figure}
	\includegraphics[width=\linewidth]{figures/snowman}
	\caption{Topological correctness of the reconstructed surface in multi-view reconstruction. The erroneous inner structures of IDR are indicated by the artifact in the image rendered by Blender~\cite{Hess:2010:BFE:1893021} (using glossy and transparent material, and show back face) and the contours of signed distance field the at cross-sections.}\label{fig:dtu}
\end{figure}
IDR impressive geometry details on the DTU dataset~\cite{jensen2014large}, but a closer inspection shows that the reconstructed surface contains many topological errors inside visible surface.
We show iso-points can be utlized to improve the topological accuracy of the reconstructed surface.

We use the same network architecture and training protocol as IDR, which samples 2048 pixels from a randomly chosen view in each optimization iteration.
Uniform iso-points are used in this experiment.
In order to keep similar sample count, we subsample the visible iso-points to obtain a maximum of 1500 on-surface samples per iteration.
Since our strategy automatically creates more in-surface samples (as shown in Figure~\ref{fig:ray-march}), we reduce the loss weight on the in-surface samples to 20\% of the original implementation.

We visualize the topology of the reconstructed surface in Figure~\ref{fig:dtu}.
To show the inner structures of the surface, we render the surface in transparent material with a physically-based renderer.
Dark patches in the rendered images reflect erroneous light transmission caused by inner structures \yf{Shihao proof read}. 
Similarly, we also show the contours lines of the iso-surface on a cross-section.

In both visualizations, the incorrect topology in IDR reconstruction is clearly visible. 
In comparison, our sampling enables more accurate reconstruction of the signed distance field inside and outside the surface.

\subsection{Regularizing with iso points}
In this section, we evaluate the benefit of using iso-points for regularization.
As a example application, we consider surface reconstruction from noisy point cloud.

We use the Furu~\cite{furukawa2009accurate} reconstruction of the DTU dataset as the input.
As the baseline, we use the publicly available SIREN codebase and adopt their default optimization protocol for 3D surface fitting.
Given a dense point cloud with normals scaled to a unit cube, in each optimization iteration the baseline method samples an equal number of surface points and off-surface points from the point cloud and randomly from a unit cube respectively as training points.
Denoting the surface points as $ \Q_s = \{\q_s, \n_s\} $ and the off-surface points as $ \Q_o = \{\q_o, \n_o\} $, the optimization objective is made of four parts:
$ \mathcal{L} = \gamma_{\text{onSDF}}\mathcal{L}_{\text{onSDF}} +  \gamma_{\text{normal}}\mathcal{L}_{\text{normal}} +\gamma_{\text{offSDF}}\mathcal{L}_{\text{offSDF}}+\gamma_{\text{eikonal}} \mathcal{L}_{\text{eikonal}} $, where
{\scriptsize
	\[ \mathcal{L}_{\text{onSDF}} = \frac{\sum_{\q_s\in \Q_s}|f(\q_s)|}{|\Q_s|}, \, \mathcal{L}_{\text{normal}} = \frac{\sum_{\q_s\in \Q_s}|1-\cos(J_f^T(\q_s), \n_s)|}{|\Q_s|}, \]
	\[ \mathcal{L}_{\text{offSDF}} = \frac{\sum_{\q_o\in \Q_o}e^{-\alpha|f(\q_o)|}}{|\Q_o|}, \, \mathcal{L}_{\text{eikonal}} = \frac{\sum_{\q\in \Q_o\cup\Q_s }|1-\|J_f^T(\q)\||}{|\Q_s|+|\P_o|} \].
}

We alter this objective with the outlier-aware loss weight in \eqref{eq:outlier_weight} and additionally add the regularizations on iso-points \eqref{eq:iso_sdf} and \eqref{eq:iso_normal}.
\ie
{
	\scriptsize
\begin{align*}\label{eq:onsurface_weight}
	\mathcal{L}_{\text{onSDF}} &= \frac{\sum_{\q_s\in \Q_s}v(\q_s)|f(\q_s)|}{|\Q_s|}, \\
	\mathcal{L}_{\text{normal}} &= \frac{\sum_{\q_s\in \Q_s}v(\q_s)|1-\cos(J_f^T(\q_s), \n_s)|}{|\Q_s|}. 
\end{align*}
}

%\paragraph{Comparision of different regularizations.}

\begin{figure}
\includegraphics[width=\linewidth]{figures/owl}
\caption{Implicit surface reconstruction from noisy and incomplete point cloud. From left to right: input, results of Poisson surface reconstruction, SIREN, and ours. Our method is based on SIREN but we improve it by using our adaptive sampling to regularize the optimization process. \yf{Add one or two more examples. also add point2surf. put evaluation next to owl model. Rename SIREN to direct optimization.}}\label{fig:owl}
\end{figure}


\subsection{Performance analysis}
\begin{figure}
\footnotesize\centering
\begin{tikzpicture}
	\begin{semilogyaxis}[
		height=5cm, width=\linewidth,
		xlabel=time (s),
		ylabel=chamfer distance]
		\addplot[color=red,mark=x] 
		table[x=mtime,y=chamfer_p,col sep=comma,comment chars=\#] {data/compressor_implicit.log};
		\addplot[color=brown,mark=o] 
		table[x=mtime,y=chamfer_p,col sep=comma,comment chars=\#] {data/compressor_uni.log};		
		\addplot[color=teal,mark=triangle] 
		table[x=mtime,y=chamfer_p,col sep=comma,comment chars=\#] {data/compressor_curvatureS.log};		
		\addplot[color=blue,mark=x] 
		table[x=mtime,y=chamfer_p,col sep=comma,comment chars=\#] {data/compressor_lossS.log};
		\legend{vanilla ray tracing, ours uniform, ours loss-aware}
	\end{semilogyaxis}
\end{tikzpicture}
\caption{Chamfer distance}
\end{figure}
